Searches for small-scale anisotropies from neutrino point sources with three years of IceCube data

Recently, IceCube found evidence for a diffuse signal of astrophysical neutrinos in an energy range of $60\,\mathrm{TeV}$ to the $\mathrm{PeV}$-scale. The origin of those events, being a key to understanding the origin of cosmic rays, is still an unsolved question. So far, analyses have not succeeded to resolve the diffuse signal into point-like sources. Searches including a maximum-likelihood-ratio test, based on the reconstructed directions and energies of the detected down- and up-going neutrino candidates, were also performed on IceCube data leading to the exclusion of bright point sources. In this paper, we present two methods to search for faint neutrino point sources in three years of IceCube data, taken between 2008 and 2011. The first method is an autocorrelation test, applied separately to the northern and southern sky. The second method is a multipole analysis, which expands the measured data in the northern hemisphere into spherical harmonics and uses the resulting expansion coefficients to separate signal from background. With both methods, the results are consistent with the background expectation with a slightly more sparse spatial distribution, corresponding to an underfluctuation. Depending on the assumed number of sources, the resulting upper limit on the flux per source in the northern hemisphere for an $E^{-2}$ energy spectrum ranges from $1.5 \cdot 10^{-8}\,\mathrm{GeV}/(\mathrm{cm}^2 \mathrm{s})$, in the case of one assumed source, to $4 \cdot 10^{-10} \,\mathrm{GeV}/(\mathrm{cm}^2 \mathrm{s})$, in the case of $3500$ assumed sources.

==> data_analysis.tex <==
\section{Data Analysis}
\subsection{Discovery Potential of the autocorrelation test}
The signal injection is divided into different steps. First, the sources are randomly distributed over the sky according to the specific scenario. In a second step, the detector acceptance is taken into account and the signal events are distributed around the sources, according to their specific angular resolution. This angular resolution is obtained from the Point Spread Function (PSF) of each signal event from Monte Carlo events and is shown on Figure \ref{psf}. Then, the events get inserted into the background events, while for every injected signal event one background event similar in declination is erased. This procedure is done to keep the total number of events fixed. In a last step the thresholds for the energy bins are re-calculated for keeping the number of events fixed in every energy bin as well.

Figure \ref{limit_north} presents the $5\sigma$ discovery potential for sources with $E^{-2}$ neutrino spectra as a function of the number of sources. The first signal model considered here were sources with equal strength and a uniform distribution across the northern sky. 
%The detector acceptance was taken into account and the total number of events in the sample was kept constant in the signal simulation. 
The second scenario is a spatial distribution according to the Green catalogue \cite{Green} of SNRs in the Milky Way and exhibits a larger clustering between the sources compared to the first scenario. The figure shows that the discovery flux per source decreases with the number of sources in both scenarios. If there are more than 50 sources of the same strength in the northern sky, this analysis is able to detect a signal that the standard likelihood point source analysis \cite{all_sky} would not see. While a discovery of a population of sources with an $E^{-2}$ neutrino spectrum is already excluded by a search for a diffuse neutrino flux in the 59-string data \cite{diffuse}, this analysis will be able to provide valuable information should a diffuse flux emerge in the future. %Since it uses a data-driven background estimation, it is more robust against systematic uncertainties. Furthermore, it might eventually unveil the first hint for a clustering in such a signal.

\subsection{Discovery Potential of the Multipole Analysis}

\subsection{Analysis Performance}
By calculating the test statistic for mixed sky maps containing only a small fraction of signal events and mainly background events, the analysis performance can be estimated. This is done by varying the number of sources $N_{\mathrm{Sou}}$ for fixed values of $\mu$ and $\gamma$. Afterwards, the resulting test statistic for each combination of $(N_{\mathrm{Sou}},\, \mu, \, \gamma)$ is calculated 1000 times and 10\,000 times for the background distribution. Exemplarily, the resulting test statistics for $\mu=5$ are shown in figure \ref{} for an $E^{-2}$ energy spectrum and various values of $N_{sou}$. Finally, the resulting sensitivity is determined by finding the number of sources needed to shift the median of the test statistic beyond the 90\%-quantile of the background distribution.

\begin{figure*}[t]
 \centering
 \subfigure[$D_{\mathrm{eff}}^{2}$ from MC simulations]{\includegraphics[width=0.48\textwidth]{plots/thesis3_effD2_mu5_E2.png}\label{fig:TS_MC}}
 \subfigure[Experimental $D_{\mathrm{eff}}^{2}$]{\includegraphics[width=0.48\textwidth]{plots/thesis2_EXP_effD2.png}\label{fig:TS_EXP}}
 \caption{(a) Test statistic shown for various amounts of signal in the expanded sky map, given by $\mu=5$, $\gamma=2$ and various values for $N_{\mathrm{Sou}}$. A Gaussian fit is shown for all cases, which is in good agreement with each distribution. (b) Test statistic for pure background compared to the experimentally observed value.}
 \end{figure*}


By using the known energy-dependent effective area $A_{\mathrm{eff}}(E)$ of the detector for the three-years sample, the resulting sensitivity in terms of signal neutrinos can be converted to fluxes. This is done using 
\begin{equation} \label{eq:Numbers2Fluxes}
E^{\gamma}\frac{\mathrm{d}\phi}{\mathrm{d}E} =  \frac{n_{\mathrm{sig}}}{ T_{\mathrm{up}} \int\limits_{0}^{\infty} \mathrm{d}E \, A_{\mathrm{eff}}(E)E^{-\gamma} } \mathrm{,}
\end{equation}
where $n_{\mathrm{sig}}$ is the number of signal neutrinos fixed by the signal parameters $(N_{\mathrm{Sou}},\, \mu, \, \gamma)$ and $T_{\mathrm{up}}$ is the detector uptime of the three-years data sample. The resulting discovery potentials for $E^{-2}$, $E^{-2.25}$ and $E^{-3}$ are shown in figure \ref{limit_north} - \ref{limit_e225}.
